A Unified Theory of Dual-Process Control

Dual-process theories play a central role in both psychology and neuroscience, figuring prominently in fields ranging from executive control to reward-based learning to judgment and decision making. In each of these domains, two mechanisms appear to operate concurrently, one relatively high in computational complexity, the other relatively simple. Why is neural information processing organized in this way? We propose an answer to this question based on the notion of compression. The key insight is that dual-process structure can enhance adaptive behavior by allowing an agent to minimize the description length of its own behavior. We apply a single model based on this observation to findings from research on executive control, reward-based learning, and judgment and decision making, showing that seemingly diverse dual-process phenomena can be understood as domain-specific consequences of a single underlying set of computational principles.

==> figures.tex <==



\begin{figure}[t]
	\begin{center}
		\includegraphics[width=14.5cm]{MDL-C_eLife/figures/Figure1.pdf}
	\end{center}
	\vspace{-2em}
	\caption{A. Schematic of a neural network implementation of MDL-C. Perceptual observations (input \textit{o} to units on the far left) feed into two recurrent networks. The lower pathway, $RN\!N_{\pi_0}$, contains noisy synaptic connections subject to VDO regularization as described in the main text. This network outputs an action distribution $\pi_0$. The upper pathway, $RNN_\pi$, outputs a separate action distribution $\pi$, which overwrites $\pi_0$, the KL divergence between the two policy outputs is computed, and an action \textit{a} is selected from $\pi$. Arrows indicate all-to-all projections. Not shown is a gating layer between input features and $RN\!N_{\pi_0}$, which was included for intepretability of results. See Methods for this and all other implementational details. B. MDL regularization enhances generalization. Left: Two agents, an MDL-C agent and an unregularized baseline (\textit{Standard RL}), were trained to navigate within a partitioned grid (inset) to a set of cued goal locations (blue tiles). In a second phase of training, the remaining (white) locations were presented as goals. The barplot shows the average number of trials elapsed before the agent first discovered a shortest path to goal. Individual points here and in subsequent figures are based on data from independent simulation runs. See Methods for details. Right: Average reward in a continuous control (running) task. MDL-C learns faster if the agent has previously encountered related tasks, and learns faster than a comparison agent lacking MDL-C's complexity penalty (\textit{Standard RL}; see Methods). Error bands here and in subsequent figures indicate standard error. In these and subsequent comparisons, unless otherwise noted, reported effects  were confirmed by rank-sum test at a threshold of p = 0.05 (see Methods).
	}
	\label{fig:fig1}
	\vspace{-1em}
\end{figure}



\begin{figure}[t]
	\begin{center}
		\includegraphics[width=12cm]{MDL-C_eLife/figures/Figure2.pdf}
	\end{center}
	\vspace{-2em}
	\caption{A. \cite{hartley2003well} reported greater activity in dorsolateral PFC (red) during wayfinding than during following of a familiar route, with the opposite effect in more posterior regions (blue). B. \cite{ciaramelli2008role} reported that damage to another (orbitofrontal) region of PFC impaired navigation to novel goals, both in the laboratory and an ecological study. In unsuccessful trials patients frequently navigated to familiar goal locations. Performance improved when patients were given frequent reminders of the goal or were asked to verbally rehearse the goal, but not when the goal reminder was replaced by an uniformative stimlus (\textit{Warning}). C. By inserting a gating layer over input features within $RN\!N_{\pi_0}$ (see Methods), we can directly read out which information is processed by that pathway. The plot shows attention weights for the three input features in the navigation task referenced in Figure 1. Over the course of the initial training block, $RN\!N_{\pi_0}$ learns to ignore the current goal cue. D. In a modified navigation task only two goals were cued, one (blue \textit{G}) occurring more frequently during training than the other (red \textit{G}). When the infrequent goal is cued at test, the intact MDL-C agent navigates successfully to it from any start state (see blue example trajectories). When $RNN_{\pi}$ is ablated, the agent ignores the instruction cue and navigates to the more frequent goal (pink trajectories). See Methods for simulation details. 
	}
	\label{fig:fig2}
	\vspace{-1em}
\end{figure}


\begin{figure}[t]
	\begin{center}
		\includegraphics[width=12cm]{MDL-C_eLife/figures/Figure3.pdf}
	\end{center}
	\vspace{-2em}
	\caption{A. Consistent with many other findings, \cite{tsuchida2013core} reported an association between damage to dorsolateral PFC and Stroop interference. B. When the MDL-C agent is trained on the Stroop task (see Methods), $RN\!N_{\pi_0}$ learns to ignore both the task cue and the stimulus color, attending only to word identity. C. Policies for $RN\!N_{\pi}$ (top) and $RN\!N_{\pi_0}$ (bottom) for the stimuli shown, in word-reading (\textit{WR}) and color-naming (\textit{CN}) contexts. Response probabilities are shown for the response \textit{red}, complementary to (unshown) probabilities for the alternative \textit{blue} response.  D. Left: KL divergence between $\pi$ and $\pi_0$ for the four trial types shown in panel C. Right: Corresponding reaction times (see Methods). E. When trained on the Stroop task and then given a choice between blocks of color-naming trials that involve either high or low proportions of incongruent stimuli (see Methods), the MDL-C agent displays a preference for less frequent incongruence, paralleling the demand-avoidance effect seen in human decision making.   
	}
	\label{fig:fig3}
	\vspace{-1em}
\end{figure}



\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=10cm]{MDL-C_eLife/figures/Figure4redux.pdf}
	\end{center}
	\vspace{-2em}
	\caption{MDL-C minimizes the description length of its own behavior. In each plot, the x axis tracks the multiplicative weight placed on the complexity term in the MDL objective during training (see Methods). The y axis shows the KL costs, expressed in natural units of information (nats), corresponding to the deviation term in the MDL-C objective (blue), the complexity term (pink) and their unweighted sum (black). The complexity term naturally falls with increases to the weight placed on the complexity penalty during training. At the same time, this reduction in complexity causes the policy $\pi_0$ to diverge from the policy $\pi$, progressively inflating $D_{KL}(\pi || \pi_0)$. Note that the KL sum is the quantification of the full description length that applies when the complexity cost weight is 1.0 (see Methods and Supplementary Discussion). As shown, this measure displays a U-shaped profile with a minimum at 1.0. MDL-C thus minimizes the description length of behavior, as quantified within the objective function employed for training. Panels A-D illustrate the effect for our simulations of the Stroop task (A); navigation as referenced in Figure 1 (B); the two-step task (C); and the multiattribute decision-making task from Simulation 3, in the parameter regime producing behavior as in Figure 6D (D).
	}
	\label{fig:fig4}
	\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=12.0cm]{MDL-C_eLife/figures/fig5_elife.pdf}
	\end{center}
	\vspace{-2em}
	\caption{\textbf{A}. In line with many other pieces of evidence, \cite{glascher2010states} reported a functional-anatomical dissociation between signals related to model-based RL, in dorsolateral PFC (orange), and signals related to model-free RL (green). \textbf{B}. Structure of the two-step task as introduced by \cite{daw2011model}. Choice occurs at Stage 1. The value of \textit{p} varies over time, and so must be inferred by the participant. Following subsequent research, the version employed in our experiments additionally included explicitly cued reversals in the structure of transitions from Stage 1 to Stage 2. See Methods for full details. \textbf{C}. Classical behavioral signatures of model-free (left) and model-based (center) performance in the two-step task. Adapted from \cite{miller2016identifying}, the plots show logistic regression weights quantifying the influence of two factors on the probability of repeating on the index trial the same first-stage action selected on the previous trial: (1) whether reward was received or omitted on the previous trial, and (2) whether the previous trial featured a transition from stage 1 to 2 that was high-probability (\textit{common}) or low (\textit{uncommon}). The right panel shows a hybrid pattern, similar to that reported in the classic study by \citep{daw2011model}. \textbf{D}. Left: Two-step behavior of MDL-C, reflecting policy $\pi$. Right: Influence of the past on policy $\pi_0$. %E. Logistic regression weights describing influence on current-trial Stage 1 choice (stay probability) of outcomes on preceding five trials, for $\pi$ (left) and $\pi_0$ (right). Patterns match respectively those previously described for model-based and model-free behavior (see Methods for discussion). 
	\textbf{E}. Same as Panel D but with different weighting of terms in the MDL-C objective (see Methods and compare panel C, right). \textbf{F}. Logistic regression weights showing the influence on the current action of reward contingent on choice (reward seeking), previous choices (perseveration), and reward independent of choice (main effect of outcome) of MDL-C and a standard RL agent on the drifting two-armed bandit task from \cite{miller2018predictive}. MDL-C displays a stronger tendency towards perseveration, reminiscent of rats trained on the same task. \textbf{G}. Left: Simulation of contingency degradation from \cite{miller2019habits}. The longer the training phase (x axis), the longer lever-pressing persists after reward is discontinued (red). Right: Corresponding behavior from MDL-C, also showing the effect of ablating $\pi_0$.
	}
	\label{fig:fig5}
	\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=12cm]{MDL-C_eLife/figures/Figure6.pdf}
	\end{center}
	\vspace{-2em}
	\caption{A. \cite{de2011heuristics} reported elevated activity in dorsolateral PFC when participants overrode heuristic-based responses to engage in richer reasoning. Image displays region of interest, drawn from \cite{goel2000dissociation}. B. Heuristic one-reason decision making (left) and richer compensatory decision making (right) in a multi-attribute choice task, from \cite{binz2022heuristics}. Gini coefficients, on the y axis, capture the degree to which decisions depend on one feature (higher values, with asymptotic maximum of one) versus all features evenly (zero), with references for one-reason decision making (\textit{single cue}) and a fully compensatory strategy (\textit{equal weighting}) indicated. Data points for each trial correspond to observations from separate simulation runs. Human participants in the study displayed both patterns of behavior, depending on the task conditions. C. Behavior of MDL-C in the task from \cite{binz2022heuristics}, under conditions where human participants displayed one-reason decision making. D. Behavior of $\pi_0$ (left) and $\pi$ (right) when the KL penalty for divergence between the two policies is reduced (see Methods). E. In the simulation from panel D, the divergence between policies is increased when the agent emits a non-heuristic decision. 
	}
	\label{fig:fig6}
	\vspace{-1em}
\end{figure*}


\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=10cm]{MDL-C_eLife/figures/Figure7.pdf}
	\end{center}
	\vspace{-2em}
	\caption{\textbf{A.} Top: Behavioral data from the modified Stroop task studied by \cite{cm1988training}. Early in training, shape-naming responses were  both slower than color-naming responses and more affected by stimulus congruence, consistent with shape-naming being the relatively 'controlled' response and color-naming relatively 'automatic.' With extensive training, the pattern flipped, with shape-naming becoming faster than color-naming and less affected by stimulus congruence.  Bottom: Under training conditions mimicking the experimental study, MDL-C displayed a similar pattern of behavior, with a significant main effect of task and a significant interaction between task and trial-type (p < 0.05) at both 0 trials and 44,000 trials. \textbf{B.} Zero-shot Stroop performance in MDL-C and an unregularized baseline model (see Methods). Top: Color-naming accuracy on incongruent Stroop stimuli, after training only with neutral stimuli (see main text and Methods). Bottom: KL divergence between action probability distributions under two conditions, (1) presentation of incongruent Stroop stimuli, and (2) presentation of Stroop stimuli with the word identity input masked out. MDL-C shows significantly lower divergence, indicating that the control policy attends less to the task-irrelevant factor --- i.e., MDL-C is more robust to distractors --- despite never having been trained on incongruent stimuli.
	}
	\label{fig:fig7}
	\vspace{-1em}
\end{figure*}
